Noncontextual versus contextual interferometry

Feynman famously said that single-particle interference is ``a phenomenon which is impossible to explain in any classical way, and which has in it the heart of quantum mechanics.'' In this paper we show that some of the phenomenology of interference can be reproduced in a ``classical'' way, by reproducing the Elitzur-Vaidman Bomb Tester (including their improved version) using an extension of the quantum simulation logic (QSL) formalism. Our result improves and simplifies a previous result by Catani \emph{et al}, which relies on a much more complicated extension involving a ``toy field theory.'' We also show that not all single-particle interference can be explained by such a simple extension (including that of Catani et al), by showing that Hofmann's three-path interferometer is ``nonclassical'' in a very specific sense: it violates a Kochen-Specker-noncontextual inequality. Given that both our extension of QSL and Catani et al's extension are \emph{noncontextual} -- so do not reproduce the contextual behaviour of Hofmann's three-path interferometer -- the behaviour of that interferometer is a proper example of a phenomenon that has in it the heart of quantum mechanics, according to Feynman.

==> tikzlibraryqcircuit.code.tex <==
% tikzlibraryqcircuit
% -*- mode: LaTeX -*-
%
% Simple drawing of quantum circuits
%
%
% Version 1.2 <jan-ake.larsson@liu.se> 2015-06-30
%
% Copyright 2015 Jan-AAke Larsson

\usetikzlibrary{matrix}% Placement of gates in qcircuit
\usetikzlibrary{fit}% Multiple-bit unitary = mgate
\usetikzlibrary{shapes.misc}% Shape "cross out" = swap
\usetikzlibrary{shadows.blur}
\pgfdeclarelayer{qcircuit}%
\pgfsetlayers{qcircuit,main}%
\definecolor{gatecolor}{rgb}{0.97,0.97,.97}
\tikzset{%	
  gateshadow/.style={shadow yshift=-2pt, shadow xshift=2pt, opacity=0.3},
  qcircuit/.style={matrix of math nodes,nodes in empty cells=true,%
    nodes={anchor=center,inner sep=0pt,minimum size=1.5em,%
      % Gives the last cell in each row the alias qc0_end, qc1_end, ...
      alias=qc\the\pgfmatrixcurrentrow_end,
      },%
    column 1/.style={nodes={
      % Gives the first cell in each row the alias qc0, qc1, ...
      alias=qc\the\pgfmatrixcurrentrow,
      }},
    column sep=3mm,row sep=1mm},%
  gate/.style = {draw,fill=gatecolor,inner sep=1mm,minimum size=1.5em,drop shadow=gateshadow},%
  nsgate/.style = {draw,fill=gatecolor,inner sep=1mm,minimum size=1.5em},%
  mgate/.style = {draw,fill=gatecolor,drop shadow=gateshadow,inner sep=0pt,fit=#1,
    %%%%%%%%%%%%%%% Needed to correct node text vertical alignment in fitted node
    %%%%%%%%%%%%%%% Is this a bug in tikz fit library?
    %%%%%%%%%%%%%%% Fix from http://tex.stackexchange.com/questions/79172/wrong-vertical-text-position-with-tikz
    text height/.expanded=\the\pgf@y+.5\ht\pgfnodeparttextbox
    -.5\dp\pgfnodeparttextbox
    %%%%%%%%%%%%%%% End correction
  },%
  ctrl/.style = {circle,draw,fill,minimum size=4pt,inner sep=0pt},%
  ictrl/.style = {circle,draw,semithick,fill=white,%
    minimum size=5pt,inner sep=0pt},%
  swap/.style={cross out,draw,semithick,minimum size=8pt},%
  cnot/.style={circle,draw,semithick,fill=white,minimum size=9pt,%
    inner sep=0pt, path picture={ \draw[thick](path picture bounding
      box.north) -- (path picture bounding box.south) (path picture bounding
      box.west) -- (path picture bounding box.east); }},%
  meter/.style = {draw,fill=gatecolor,drop shadow=gateshadow,minimum size=1.5em,path picture={%
      \draw[semithick] (path picture bounding box.south) ++(0,.1em)
      ++(45:.9em) arc (45:135:.9em);%
      \draw[semithick,->] (path picture bounding box.south) ++(0,.1em)
      -- +(70:1.3em); }%
  },%
  dots/.style = {draw=white,fill=white,inner sep=3.2mm,minimum size=1.5em,path picture={\draw[semithick] node {\hspace{-.3ex} \textbf{\dots}};}
  },%
  vdots/.style = {draw=white,fill=white,inner sep=3.2mm,minimum size=1.5em,path 
  picture={\draw[semithick] node {\hspace{-.75ex} 
  \raisebox{1.4ex}{\textbf{\vdots}}};}
  },%
  ddots/.style = {draw=white,fill=white,inner sep=3.2mm,minimum size=1.5em,path 
  picture={\draw[semithick] node {\hspace{-.75ex} 
  \raisebox{1.4ex}{\textbf{$\ddots$}}};}
  }%
}

\providecommand{\ket}[1]{\ensuremath{\left|#1\right\rangle}}
\providecommand{\bra}[1]{\ensuremath{\left\langle#1\right|}}

